DisenHCN: Disentangled Hypergraph Convolutional Networks for Spatiotemporal Activity Prediction

Spatiotemporal activity prediction, aiming to predict user activities at a specific location and time, is crucial for applications like urban planning and mobile advertising. Existing solutions based on tensor decomposition or graph embedding suffer from the following two major limitations: 1) ignoring the fine-grained similarities of user preferences; 2) user's modeling is entangled. In this work, we propose a hypergraph neural network model called DisenHCN to bridge the above gaps. In particular, we first unify the fine-grained user similarity and the complex matching between user preferences and spatiotemporal activity into a heterogeneous hypergraph. We then disentangle the user representations into different aspects (location-aware, time-aware, and activity-aware) and aggregate corresponding aspect's features on the constructed hypergraph, capturing high-order relations from different aspects and disentangles the impact of each aspect for final prediction. Extensive experiments show that our DisenHCN outperforms the state-of-the-art methods by 14.23% to 18.10% on four real-world datasets. Further studies also convincingly verify the rationality of each component in our DisenHCN.

==> append.tex <==
\section{APPENDIX FOR REPRODUCIBILITY}
\subsection{Dataset Details}
\label{sec::DATASET}
For the reproducibility, we'll describe the details of data processing in this section.
\iffalse
\begin{table}[t]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
\caption{Statistics of Datasets}
\centering
%\small
\setlength\tabcolsep{1.5pt}
\scalebox{0.85}{
\begin{tabular}{ccccccc}
\toprule[1pt]
{\bf Dataset}  & \#{\bf User} & \#{\bf Location} & \#{\bf Time} & \#{\bf Activity} & \#{\bf Records} &{\bf Density}  \\
\hline
{\bf Telecom}       & 10,099 &2,462 &48 &1,751 &604,401 &2.9e-7     \\
{\bf TalkingData}   & 4,068 &1,302 &48 &2,310 &409,651 &6.9e-7     \\
{\bf 4SQ}    & 10,543 &1,585 &31 &3,973 &291,485 &1.4e-7     \\
{\bf TWEET}   & 10,414 &2,080 &27 &5,960 &333,812 &9.6e-8     \\
\bottomrule[1pt]
\end{tabular}}
\label{tab:ds}
\end{table}
\fi

\begin{itemize}[leftmargin=12pt,partopsep=0pt,topsep=0pt]
\item {\bf Telecom}~\cite{Telecom}: Each record of Telecom contains anonymized user ID, timestamp, connected cellular tower ID and its GPS location, and the used app ID. Following SAGCN~\cite{yu2020SAGCN}, we take the cellular base stations as the basic location units and utilize the widely used Voronoi diagrams~\cite{1991voronoi} to partition the city based on stations’ coordinates to get the the corresponding location ID. Moreover, we distinguish weekdays and weekends and discretize the time in a day into 24 units. Hence, there are 48 time slots.
\item {\bf TalkingData\footnote{\url{https://www.kaggle.com/c/talkingdata-mobile-user-demographics}}}: The pre-processing of TalkingData is almost the same as Telecom. The difference lies on the data selection.
Since records in TalkingData are distributed all around China (too large), we choose the records in Shanghai for our experiments.
\item {\bf4SQ}~\cite{crossmapwww17}: The record of 4SQ contains anonymized user ID, timestamp, longitude and latitude, and text message. We use the hotspot detection methods in CrossMap~\cite{crossmapwww17} to generate the spatiotemporal hotspots (to obtain location and timeslots ID) and keywords. Note that we regard the keywords as activities.
\item {\bf TWEET}~\cite{crossmapwww17}: The pre-processing of TWEET is almost the same as 4SQ. The difference is that we set the maximum number of keywords as 6000 in hotspot detection for efficiency.
\end{itemize}

For Telecom and TalkingData, following~\cite{yu2020SAGCN,chen2019cap}, we remove the users with less than 10 visited locations and 5 used apps. For 4SQ and TWEET, following~\cite{crossmapwww17,liu2020ACTOR}, we remove the keywords that appear less than 100 times in the entire corpus. 

The datasets statistics are summarized in Table~\ref{tab:dataset}.

\subsection{Implementation Details}
\label{sec::Imp}
All the baselines and our STHCN are implemented in Pytorch\footnote{https://pytorch.org/}. And we provide multiple settings in this section.
\subsubsection{Experiments Settings}
All experiments are conducted with the following settings:
\begin{itemize}[leftmargin=12pt,partopsep=0pt,topsep=0pt]
\item {Operating system}: Ubuntu 16.04.6 LTS
\item {CPU}: Intel(R) Xeon(R) CPU E5-2650 v4 @ 2.20GHz
\item {GPU}: Nvidia Titan Xp
\item {Software version}: Python 3.6.10; Pytorch 1.6.0; Numpy 1.19.1; SciPy 1.5.2; scikit-learn 0.23.2
\end{itemize}
\subsubsection{Baseline Settings}
We implement the baselines based on the available implementations of authors and the details in the corresponding papers. The tensor models are based on the implementations of UCLAF~\cite{zheng2010UCLAF}. As for SA-GCN~\cite{yu2020SAGCN}, we implement it referring to GCN~\cite{GCN} and the details in paper. Moreover, we adapt LightGCN~\cite{he2020lightgcn} and HGNN~\cite{feng2019HGNN} to saptiotemporal activity prediction refers to the graph construction of SA-GCN. And the codes of our STHCN is based on the pytorch implementation of LightGCN and HGNN. Finally, we list the
publicly available implementation URLs of baselines as follows:
\begin{itemize}[leftmargin=12pt,partopsep=0pt,topsep=0pt]
\item {\bf UCLAF}:\url{https://github.com/vwz/UCLAF}
\item {\bf ACTOR}:\url{https://github.com/PonderLY/ACTOR}
\item {\bf CrossMap}:\url{https://drive.google.com/open?id=0Byrzhr4bOatCck5mdWJnb2xudVk}
\item {\bf GCN}: \url{https://github.com/tkipf/pygcn}
\item {\bf LightGCN}:\url{https://github.com/gusye1234/LightGCN-PyTorch}
\item {\bf HGNN}:\url{https://github.com/iMoonLab/HGNN}
\end{itemize}
\subsubsection{Hyperparameter Settings}

In our experiments, we conduct early stopping and the same train settings for all models, which is shown in Table~\ref{tab:hyperpa}. We use early stopping to detect over-fitting, and training process will be stopped if Recall@10 or NDCG@10 on validation set does not increase for 20 epochs. The initial learning rate is 0.001, which will be decayed 0.5 in epoch 50, 100, 200, and 400. And Table~\ref{tab:hypar-model} represents the layer, embedding dimension and hidden dimension of each model. Note that LightGCN-ST and our STHCN removed the linear transformation, so the hidden dimmension doesn't exist. For all methods, we run 5 times with the same partition
and report the average results.

%\vspace{-0.2cm}

\begin{table}[ht]
\setlength\tabcolsep{3pt}
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\caption{Hyperparameter settings in the training stage.}
\centering
\scalebox{0.8}{
\begin{tabular}{c|c}
	\toprule[1pt]
	    {\bf Parameters}     &               {\bf Value}                \\ \hline
	         Epochs          &                   500                    \\
	Early stopping threshold &                    20                    \\
	 Initial learning rate   &                   1e-3                   \\
	Learning rate milestone  &           [50, 100, 200, 400]            \\
	Learning rate decay rate &                   0.5                    \\
	       Batch size        &                   2048                   \\
	  $L_2$ regularization   & Telecom,TalkingData,4SQ:3e-5; TWEET:1e-4 \\ \bottomrule[1pt]
\end{tabular}}
\label{tab:hyperpa}
\end{table}


\begin{table}[ht]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
\caption{Hyperparameter settings for different models.}
\centering
%\small
\setlength\tabcolsep{3pt}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccc}
\toprule[1pt]
{\bf Category} &{\bf Model}  & {\bf Layer} & {\bf Embedding dim.} & {\bf Hidden dim.} \\
\hline
\multirow{4}{*}{Tensor}
& SCP       & - & 64 & -  \\
& UCLAF     & - & 64 & -  \\
& MCTF      & - & 64 & -  \\
& WDGTC     & - & 64 & -  \\\hline
\multirow{4}{*}{Graph}
& CrossMap       & 1 &64 &[64]  \\
& ACTOR     & 1 &64 &[64] \\
& SA-GCN      & 2 &64 &[64, 64]  \\
& LightGCN-ST     & 3 &64 & - \\\hline
\multirow{2}{*}{Hypergraph}
& HGNN-ST       & 1 &64 &[64]  \\
& STHCN     & 1 &64 &- \\
\bottomrule[1pt]
\end{tabular}}
\label{tab:hypar-model}
%\vspace{-0.5cm}
\end{table}

% sparse
\begin{figure}[ht]
\centering
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/TalkingData_sr.pdf}}
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/TalkingData_sn.pdf}}\\
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/4SQ_sr.pdf}}
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/4SQ_sn.pdf}}\\
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/TWEET_sr.pdf}}
\subfloat{\includegraphics[width=0.49\columnwidth]{figs/TWEET_sn.pdf}}
%\setlength{\abovecaptionskip}{-0.2cm}
%\setlength{\belowcaptionskip}{-0.cm}
\caption{Performance with different data sparsity on TalkingData, 4SQ and TWEET.} 
\label{fig::other_s}
%		\vspace{-0.4cm}
\end{figure}

\begin{figure}[ht]
		\centering
		\subfloat[TalkingData]{\includegraphics[width=0.49\columnwidth]{figs/TalkingData_lamda.pdf}}
		\subfloat[4SQ]{\includegraphics[width=0.49\columnwidth]{figs/4SQ_lamda.pdf}}
		%\setlength{\abovecaptionskip}{-0.2cm}
        %\setlength{\belowcaptionskip}{-0.cm}
		\caption{Impact of $L_2$ regularization coefficient $\lambda$.} 
		\label{fig::lambda_a}
%		\vspace{-0.4cm}
\end{figure}

\begin{figure}[ht]
		\centering
		\subfloat[TalkingData]{\includegraphics[width=0.49\columnwidth]{figs/TalkingData_L.pdf}}
		\subfloat[4SQ]{\includegraphics[width=0.49\columnwidth]{figs/4SQ_L.pdf}}
		%\setlength{\abovecaptionskip}{-0.2cm}
        %\setlength{\belowcaptionskip}{-0.cm}
		\caption{Impact of the depth of STHCN $L$.} 
		\label{fig::layer_a}
%		\vspace{-1cm}
\end{figure}

\subsection{Additional Results}
\label{sec::addexp}

In this section, we provide the additional results of our experiments: (1) the study of data sparsity on TalkingData, 4SQ and TWEET; (2) hyper-parameter ($L_2$ regularization coefficient and model depth L) study on TalkingData and 4SQ.

\subsubsection{Impact of Data Sparsity}

Following the setting in Section~\ref{sec::sparse}, we provide the additional model performance with different data sparsity on other three datasets in Fig.~\ref{fig::other_s}. We can observe that the performance gap between STHCN and other
methods becomes larger when data become sparser, which verifies that our STHCN can alleviate data sparsity issue.

\subsubsection{Hyper-parameter Study}

We give additional studuy of $L_2$ regularization coefficient $\lambda$ and number of layers L in Fig.~\ref{fig::lambda_a} and Fig.~\ref{fig::layer_a}, respectively. Consistent with the previous conclusion in Section~\ref{sec:hyperpara}, with the
increase of $\lambda$, the performance of STHCN raise first and will drop quickly if $\lambda$ is larger than $3e^{-4}$ for TalkingData and 4SQ in Fig.~\ref{fig::lambda_a}. According to Fig.~\ref{fig::layer_a}, STHCN also achieves the best performance with only one layer on TalkingData and 4SQ.

\subsection{Computation Details}
\label{sec::Computation}
In this section, we provide the computation details of equivalent efficient hypergraph convolution operation in Section~\ref{sec::multichannel-conv}. 

First, we have three interaction matrices ${\bf R_{ul}},{\bf R_{ut}},{\bf R_{ua}}$ for user's preference of location, time and activity, respectively. {\em Separate Patterns} reveal the semantics that users have similar preference of location, time and activity. Thus, we have ${{\bf H}_1}={\bf R_{ul}}, {{\bf H}_2}={\bf R_{ut}}, {{\bf H}_3}={\bf R_{ua}}$. With the equivalent matrices defined as ${\bf A}={\bf H}{{\bf H}^\top}$, we can calculate the equivalent matrices of $\mathcal P_1-\mathcal P_3$ as follows,\\
\vspace{-0.2cm}
\begin{equation}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\begin{split}
&{\bf A}_1=\bf H_1{H_1}^\top=\bf R_{ul}{R_{ul}}^\top, \\
&{\bf A}_2=\bf H_2{H_2}^\top=\bf R_{ut}{R_{ut}}^\top, \\
&{\bf A}_3=\bf H_3{H_3}^\top=\bf R_{ua}{R_{ua}}^\top.
\end{split}
\label{eqn::A1-3}
\end{equation}
Moreover, consider the example in Fig.~\ref{fig::MultiChannel} (a), user $u_1$ performed activity $a_1$ on location $l_1$ at time $t_1$, so we have ${{\bf H}_1}_{u_1l_1}={{\bf H}_2}_{u_1t_1}={{\bf H}_3}_{u_1a_1}=1$, and ${{\bf H}_7}_{u_1(l_1t_1a_1)} = {{\bf H}_1}_{u_1l_1}{{\bf H}_2}_{u_1t_1} {{\bf H}_3}_{u_1a_1}=1$, where $(l_1t_1a_1)$ is a combination instance (hyperedge) in $\mathcal P_7$. That is, we can use multiplication to represent Logical \texttt{AND} operator ($\&$) and obtain the logical relations among channels. For the given users $u_1, u_2$, the corresponding element in $A_7$ is,\\
\vspace{-0.3cm}
\begin{align}
\setlength{\abovedisplayskip}{-0pt}
\setlength{\belowdisplayskip}{-0pt}
    {{\bf A}_7}_{u_1u_2} =& [\sum\nolimits_{i=1}^{N_L}\sum\nolimits_{j=1}^{N_T}\sum\nolimits_{k=1}^{N_A} {{\bf H}_7}_{{u_1}(l_i t_j a_k)}] \times \nonumber\\
    &[\sum\nolimits_{i=1}^{N_L}\sum\nolimits_{j=1}^{N_T}\sum\nolimits_{k=1}^{N_A} {{\bf H}_7}_{{u_2}(l_i t_j a_k)}]\nonumber\\
     =&[(\sum\nolimits_{i=1}^{N_L} {{\bf H}_1}_{{u_1}{l_i}})(\sum\nolimits_{j=1}^{N_T} {{\bf H}_2}_{{u_1}{t_j}})(\sum\nolimits_{k=1}^{N_A} {{\bf H}_3}_{{u_1}{a_k}})] \times \nonumber\\
     &[(\sum\nolimits_{i=1}^{N_L} {{\bf H}_1}_{{u_2}{l_i}})(\sum\nolimits_{j=1}^{N_T} {{\bf H}_2}_{{u_2}{t_j}})(\sum\nolimits_{k=1}^{N_A} {{\bf H}_3}_{{u_2}{a_k}})] \nonumber\\
     =&[(\sum\nolimits_{i=1}^{N_L}{{\bf H}_1}_{{u_1}{l_i}})(\sum\nolimits_{i=1}^{N_L} {{\bf H}_1}_{{u_2}{l_i}})] \times \nonumber\\
     &[(\sum\nolimits_{j=1}^{N_T}{{\bf H}_1}_{{u_1}{t_j}})(\sum\nolimits_{j=1}^{N_T} {{\bf H}_1}_{{u_2}{t_j}})] \times \nonumber\\
     &[(\sum\nolimits_{k=1}^{N_A}{{\bf H}_1}_{{u_1}{a_k}})(\sum\nolimits_{k=1}^{N_A} {{\bf H}_1}_{{u_2}{a_k}})] \nonumber\\
     =& {{\bf A}_1}_{u_1u_2}{{\bf A}_2}_{u_1u_2}{{\bf A}_3}_{u_1u_2}.
\label{eqn::Aii_a}
\end{align}%
And the matrix form is denoted as follows,
\begin{equation}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
{\bf A}_7={\bf A}_1\odot{\bf A}_2\odot{\bf A}_3=(\bf R_{ul}{R_{ul}}^\top)\odot(\bf R_{ut}{R_{ut}}^\top)\odot(\bf R_{ua}{R_{ua}}^\top).
\label{eqn::A7}
\end{equation}
Similarly, with $\bf A_1, A_2, A_3$, we can calculate $\bf A_4, A_5,A_6$ as follows,\\
\vspace{-0.2cm}
\begin{equation}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\begin{split}
&{\bf A}_4={\bf A}_1\odot{\bf A}_2=(\bf R_{ul}{R_{ul}}^\top)\odot(\bf R_{ut}{R_{ut}}^\top), \\
&{\bf A}_5={\bf A}_1\odot{\bf A}_3=(\bf R_{ul}{R_{ul}}^\top)\odot(\bf R_{ua}{R_{ua}}^\top), \\
&{\bf A}_6={\bf A}_2\odot{\bf A}_3=(\bf R_{ut}{R_{ut}}^\top)\odot(\bf R_{ua}{R_{ua}}^\top).
\end{split}
\label{eqn::A4-6}
\end{equation}
In this way, we get the equivalent matrices of $\mathcal P_1-\mathcal P_7$. Further, we combine the above equivalent matrices to get the equivalent matrices of hypergraphs in {\em Separate, Local, Global} channels ${\bf A}_s,{\bf A}_l,{\bf A}_g$, according to Eq.~\eqref{eqn::mul-channel}, calculated as follows,
\begin{equation}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\begin{split}
&{\bf A}_s=({\bf H}_1\|{\bf H}_2\|{\bf H}_3){({\bf H}_1\|{\bf H}_2\|{\bf H}_3)}^\top=\sum\nolimits_{i=1}^3{\bf A}_i, \\
&{\bf A}_l=({\bf H}_4\|{\bf H}_5\|{\bf H}_6){({\bf H}_4\|{\bf H}_5\|{\bf H}_6)}^\top=\sum\nolimits_{i=4}^6{\bf A}_i, \\
&{\bf A}_g=\bf H_7{H_7}^\top={\bf A}_7.
\end{split}
\label{eqn::A1-3}
\end{equation}

With above calculation, we can easily simplify the hypergraph convolution with corresponding equivalent matrices according Eq.~\eqref{eqn::eq_conv}. In this way, we solve the problem of tremendous computational cost in hypergraph construction and perform hypergraph convolution in a more efficient way.


